Internal structure of gauge-invariant Projected Entangled Pair States

Projected entangled pair states (PEPS) are very useful in the description of strongly correlated systems, partly because they allow encoding symmetries, either global or local (gauge), naturally. In recent years, PEPS with local symmetries have increasingly been used in the study of non-perturbative regimes of lattice gauge theories, most prominently as a way to construct variational ansatz states depending only on a small number of parameters and yet capturing the relevant physical properties. For the case of one-dimensional PEPS (Matrix Product States - MPS) a bidirectional connection was established between the internal structure of the tensor network, i.e. the mathematical properties of the constituent tensors, and the symmetry. In higher dimensions this has only been done for global symmetries, where in the local (gauge) case it is known only how to construct gauge-invariant states, but not what the symmetry implies on the internal structure of the PEPS. In the present work we complete this missing piece and study the internal structure of projected entangled pair states with a gauge symmetry. The PEPS we consider consist of matter and gauge field tensors placed on the vertices and edges, respectively, of arbitrary graphs.

==> figures/tikz-setup.tex <==
\usetikzlibrary{
  positioning,
  intersections,
  arrows.meta,
  patterns,
  decorations.markings,
  decorations.pathreplacing,
  backgrounds,
  calc
}
\tikzset{
  x = 1.4em, y = 1.4em,
  tensor/.style ={
    circle,
    draw,
    minimum width = .5em,
    text width = .5em,
    text height = .5em,
    minimum height = .5em,
    inner sep = 0pt,
    align = center
  },
  stensor/.style ={
    circle,
    draw,
    minimum width = .3em,
    text width = .3em,
    text height = .3em,
    minimum height = .3em,
    inner sep = 0pt,
    align = center
  },
  dtensor/.style ={
    rectangle,
    draw,
    minimum width = 1.412*.5em,
    text width = 1.412*.5em,
    text height = 1.412*.8em,
    minimum height = 1.412*.8em,
    inner sep = 0pt,
    align = center,
    rounded corners = .5*1.412*.5em
  },
  matrix/.style ={
    circle,
    draw,
    fill = .,%current text color
    inner sep = 0pt,
    minimum size = 3pt
  },
  mid arrow/.style={
    postaction={
      decorate,
      decoration={
        markings,
        mark=at position .5 with {\arrow[#1, xshift=.2em]{Latex[length=.3em]}}
      }
    }
  },
  mid bullet/.style={
    postaction={
      decorate,
      decoration={
        markings,
        mark=at position .5 with {\node [stensor, fill=white] {};}
      }
    }
  },
  empty/.style={
    inner sep = 0pt,
    minimum size = 0pt
  },
  background grid/.style={
    ultra thin,
    draw = gray,
    step = .2em,
    opacity = 0.5
  }
}
